Perspectives and potential issues in using artificial intelligence for computer science education

Since its launch in late 2022, ChatGPT has ignited widespread interest in Large Language Models (LLMs) and broader Artificial Intelligence (AI) solutions. As this new wave of AI permeates various sectors of society, we are continually uncovering both the potential and the limitations of existing AI tools. The need for adjustment is particularly significant in Computer Science Education (CSEd), as LLMs have evolved into core coding tools themselves, blurring the line between programming aids and intelligent systems, and reinforcing CSEd's role as a nexus of technology and pedagogy. The findings of our survey indicate that while AI technologies hold potential for enhancing learning experiences, such as through personalized learning paths, intelligent tutoring systems, and automated assessments, there are also emerging concerns. These include the risk of over-reliance on technology, the potential erosion of fundamental cognitive skills, and the challenge of maintaining equitable access to such innovations. Recent advancements represent a paradigm shift, transforming not only the content we teach but also the methods by which teaching and learning take place. Rather than placing the burden of adapting to AI technologies on students, educational institutions must take a proactive role in verifying, integrating, and applying new pedagogical approaches. Such efforts can help ensure that both educators and learners are equipped with the skills needed to navigate the evolving educational landscape shaped by these technological innovations.

==> figures/constructive-alignment.tex <==
% https://tikz.dev/tikz-shapes
% https://tex.stackexchange.com/questions/244376/drawing-a-triangle
% https://tex.stackexchange.com/questions/251642/draw-arrows-between-nodes-with-tikz

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
    \node (A) at (0,0) {Learning outcomes};
    \node (B) at (2,2) {Teaching and learning activities};
    \node (C) at (4,0) {Assessment};

    \draw[<->, to path={-- (\tikztotarget)}]
    (A) edge (B) (B) edge (C) (C) edge (A);
    \end{tikzpicture}
    \caption{Biggs' constructive alignment separates teaching and learning activies, learning outcomes, and assessment while considering them as interrelated entities \cite{biggs2022teaching}}
    \Description{The corners of the triangle have been connected using bidirectional arrows from corner to corner to show how the aspects are interrelated.}
    \label{fig:constructive-alignment}
\end{figure}

